Constrained Low-rank Matrix Estimation: Phase Transitions, Approximate Message Passing and Applications

This article is an extended version of previous work of the authors [40, 41] on low-rank matrix estimation in the presence of constraints on the factors into which the matrix is factorized. Low-rank matrix factorization is one of the basic methods used in data analysis for unsupervised learning of relevant features and other types of dimensionality reduction. We present a framework to study the constrained low-rank matrix estimation for a general prior on the factors, and a general output channel through which the matrix is observed. We draw a paralel with the study of vector-spin glass models - presenting a unifying way to study a number of problems considered previously in separate statistical physics works. We present a number of applications for the problem in data analysis. We derive in detail a general form of the low-rank approximate message passing (Low- RAMP) algorithm, that is known in statistical physics as the TAP equations. We thus unify the derivation of the TAP equations for models as different as the Sherrington-Kirkpatrick model, the restricted Boltzmann machine, the Hopfield model or vector (xy, Heisenberg and other) spin glasses. The state evolution of the Low-RAMP algorithm is also derived, and is equivalent to the replica symmetric solution for the large class of vector-spin glass models. In the section devoted to result we study in detail phase diagrams and phase transitions for the Bayes-optimal inference in low-rank matrix estimation. We present a typology of phase transitions and their relation to performance of algorithms such as the Low-RAMP or commonly used spectral methods.

==> answer_ref <==
Answer to referee:

We agree with the referee that this is a point that appears tricky, this question often arrises and we should have commented on it in the paper. In the revised version we do. We added two paragraphs (attached below).

Additionally we updated references and corrected a couple of misprints.

Sincerely

The authors




The two paragraphs we added: 

(in AMP derivation)
It should be noted at this point that the BP algorithm is guaranteed to be exact for a general system only when the underlying graphical model is a tree. Yet it is often applied to locally-tree like graphical models. On tree-like graphical models usage of BP is justified when correlations decay fast enough so that far-away boundary of a rooted tree typically does not influence the root. This is formalized as point-to-set correlations
[65]. In the present case the graphical model is fully connected and hence a derivation based on belief propagation
might seem puzzling at the first sight. The main assumptions done in belief propagation is that the incoming messages are probabilistically independent when conditioned on the value of the root. For this to be true the underlying graphical model does not have to be tree-like it can also be because the interactions are sufficiently weak. In the present case the factor $1/\sqrt{N}$ in the Hamiltonian (1)-(2) makes the interactions sufficiently weak so that the assumption of independence of incoming messages is correct in the large size limit. This is quite a common situation known from the cavity method derivation of the solution for the Sherrington-Kirkpatrick spin glass model
[66]. The resulting equations can be derived also by other means, e.g. the Plefka expansion [67] that we use later to derive the Bethe free energy. We prefer the derivation from BP, because that is the only one we know of that provides time indices that lead to a converging algorithm (note that the TAP equations with the "naive" time indices were notoriously known not to converge even in the paramagnetic phase). 

(in conclusion)
In this paper we considered models that lead to fully connected
graphical models. It should be noted that the results and phase
diagrams derived here in this setting are expected to hold as long as
the average degree of the underlying factor graph is large enough
(goes to infinity, after the $N\to \infty$ limit has been taken). 
Such expectation was proved rigorously in some special cases, see
e.g. [44,46]. 

